SoK: Leveraging Transformers for Malware Analysis

The introduction of transformers has been an important breakthrough for AI research and application as transformers are the foundation behind Generative AI. A promising application domain for transformers is cybersecurity, in particular the malware domain analysis. The reason is the flexibility of the transformer models in handling long sequential features and understanding contextual relationships. However, as the use of transformers for malware analysis is still in the infancy stage, it is critical to evaluate, systematize, and contextualize existing literature to foster future research. This Systematization of Knowledge (SoK) paper aims to provide a comprehensive analysis of transformer-based approaches designed for malware analysis. Based on our systematic analysis of existing knowledge, we structure and propose taxonomies based on: (a) how different transformers are adapted, organized, and modified across various use cases; and (b) how diverse feature types and their representation capabilities are reflected. We also provide an inventory of datasets used to explore multiple research avenues in the use of transformers for malware analysis and discuss open challenges with future research directions. We believe that this SoK paper will assist the research community in gaining detailed insights from existing work and will serve as a foundational resource for implementing novel research using transformers for malware analysis.

==> Tables/newtable.tex <==
% \input{main.bbl}
\begin{table*}[hb!]
\centering
\caption{Malware Analysis: Comprehension of Modeling Techniques, Unique Contributions, Reason behind the Implementation and Effectiveness}
\label{Table:OthersTable}
\vspace{-3mm}
\begin{adjustbox}{width=\textwidth}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{|p{2.5cm}|p{4cm}|p{7cm}|p{9cm}|}
\hline
\rowcolor{gray!15}
\textbf{Transformer} & \textbf{Task} & \textbf{Modifications / Unique Contribution}  & \textbf{Effectiveness}\\
\hline
GPT-2 Transformer~\cite{hu2021single}	&Single-shot black-box adversarial evasion&	\textbf{Fine-tuned} GPT-2 on benign file sequences to generate benign-looking adversarial perturbations&	Created adversarial perturbations in a single query, achieving \textbf{24.51\% evasion rate} without multiple feedback loops\\
\hline
Parallel N-gram Transformer Modeling ~\cite{yang2022n}&	Detection of DGA domains&Parallel combination of the N-gram algorithm and \textbf{Transformer to enhance feature extraction}&	Parallel N-gram architecture ensures richer feature extraction achieving an \textbf{accuracy of 96.97}\%\\
\hline
% CANINE-c~\cite{gogoi2023dga}	&Detection of DGA domains& \textbf{Fine-tuned} on 1 million DGA and benign domain names&Fine-tuning the character-level processing enhances the models \textbf{accuracy to 99}\%\\
% \hline

% GenTAL, skip-gram with denoising~\cite{li2023gental}&	Unsupervised binary code similarity detection& \textbf{Pre-trained} using masked instruction recovery, \textbf{Fine-tuned}, Combines skip-gram loss, denoising autoencoder principles using the transformer &Better handles semantic variations in binary code due to different compilation options, achieved\textbf{ 0.76 and 0.74 MRR} for cross-compiler \& obfuscation detection\\
% \hline
% Hybrid LSTM Transformer~\cite{guan2021malware}&	Anomaly Detection&\textbf{Combines} LSTM and Transformer for enhanced feature extraction& Demonstrates the effectiveness for \textbf{temporal dynamics and global attention} with 1.6\% improvement compared to LSTM-based models\\
% \hline
% BERT Transformer~\cite{ghourabi2022security}&	Intrusion and Malware detection in healthcare systems&\textbf{Fine-tuned} on textual network flow data from healthcare, LightGBM for malware and intrusion detection&Hybrid approach leverages transformer and gradient-boosting to \textbf{optimize performance and memory efficiency}\\
% \hline
% Residual 1D Image Transformer~\cite{barut2022r1dit}&	Privacy-preserving malware traffic classification& Uses \textbf{1-D convolutions \& 2-D positional encoding.} Meta-learning done using transfer \& few-shot learning&	Dimensional changes \textbf{improved the feature extractions} improving the detection rate of new and unseen malware\\
% \hline
% BERT, XLNet, and ULMFiT ~\cite{shahid2020devising}&	Malware characteristic classification&\textbf{Fine-tuned} on a cybersecurity dataset&BERT and XLNET showed promise in \textbf{handling context and complexity} of malware-related sentences\\
% \hline
% Hierarchical Transformer\cite{hu2020exploit}&	IoT Malware Detection&Leverages internal information from malware with two-layer hierarchy \& \textbf{integrates multi-head attention}& Hierarchical design helps to better understand packet \& session based anomalies, \textbf{significantly improves} detection \textbf{accuracy to 98.75}\%\\
% \hline
% BERT + CNN-BiLSTM + Local Attention\cite{hamad2021bertdeep}&	Cross-architecture IoT malware detection& BERTDeep-Ware enhances feature representations, \textbf{Fine-tuned} for multiple IoT CPU architectures&Significantly \textbf{improved detection} of \textbf{complex malware behaviors} with more than 90\% accuracy\\
% \hline

% Custom model (TransMalDE)\cite{deng2023transmalde}&	IoT malware detection & Integrates Transformer, uses \textbf{location embedding} to model sensitive API subgraphs&Demonstrated \textbf{superior performance} compared to CNN, LSTM, and GRU, with over 96\% accuracy\\
% \hline
% Transformer with additive attention, residual weight parameters\cite{li2023iot}&	IoT malware threat hunting&	Improved by \textbf{replacing multi-head with additive attention}, added \textbf{residual weight parameters} to tackle vanishing gradients&Additive attention \textbf{scales linearly with the sequence length without compromising accuracy}\\
% \hline
% ViT4Mal lightweight ViT\cite{ravi2023vit4mal}&	Malware detection on edge devices&\textbf{Optimized for low resource usage}, with quantization and hardware-specific optimizations&ViT4Mal achieves \textbf{competitive accuracy with minimal layers} and attention heads and \textbf{41x speedup} compared to the original ViT\\
\hline
Adaptive Transformer (AdaTrans) with an adaptive factor\cite{piadatrans}&IoT malware detection&	AdaTrans \textbf{enhances} the standard Transformer allowing to\textbf{ weigh the importance of different semantic features}&	AdaTrans’ adaptive multi-head attention mechanism proved \textbf{highly effective in capturing subtle malware behaviors} that exploit Android’s ICC (Inter Component Communication) system\\
\hline
Vanilla Transformer\cite{wangwang2021network}&	IoT malware detection&Transformer was applied to analyze network traffic features and \textbf{enhance representations}&\textbf{Improved detection accuracy} to 99.38\% accuracy on character-level features and 99.52\% accuracy on word-level features\\
\hline
BERT based VICTORY\cite{bellante2021victory}&	IoT malware detection&BERT fine-tuned using embeddings from API calls focusing on \textbf{rapid re-training with minimal data}&	Fine-tuning with BERT helped maintain \textbf{high accuracy even with low malware sample rates}\\
\hline

Directional Graph Transformer (DGT)~\cite{moon2021directional}&Malware classification&DeepWalk algorithm converts Control Flow Graphs into sequences for Transformer to \textbf{generate embeddings}&Framework \textbf{results significant improvements in detecting malware that uses complex control flow}\\
\hline

GPT-2 ~\cite{csahin2021malware}&	Malware Detection&	\textbf{Fine-tuned} GPT-2 on assembly sequences from PE files&Fine-tuning resulted\textbf{ better accuracy} than not fine tuning\\
\hline

Vision Transformer (ViT) with Lambda Attention ~\cite{chen2022malicious}&	Malware Classification&\textbf{Replaced self-attention quadratic computations with linear Lambda Layer} by introducing positional relationship learning using $\lambda_c$ (contextual) and $\lambda_{np}$ (positional)&Lambda Layer\textbf{ reduces memory complexity} while maintaining lower resource consumption and \textbf{reducing training time by up to 30x}\\
\hline

GPT-2 with Stacked BiLSTM ~\cite{demirci2022static}&	Malware Detection&GPT-2 \textbf{fine-tuned} on assembly instructions with\textbf{ stacked BiLSTM layers} for document \& sentence-level analysis&Combination \textbf{enhances contextual understanding} and improves detection performance\\
\hline

ViT enhanced with patch encoding ~\cite{park2022vision}	&Malware Classification	&\textbf{Fine-tuned} ViT employing \textbf{data augmentation with patch encoded malware images}&	Fine-tuning helps in \textbf{capturing patterns missed by traditional models}\\
\hline
BERT, DistilBERT, AlBERT, RoBERTa ~\cite{pandya2023malware}&	Malware Classification	&Generate \textbf{context-aware} opcode embeddings&Combining contextual embeddings with Resnet-18 CNN results \textbf{applicability of transformers in conjunction with deep learning} classifiers\\
\hline

Graph Transformer with triplet loss ~\cite{bu2023triplet}&	Few-shot Malware Classification	&\textbf{Introduction of graph transformer} to embed malware control flow graphs (CFGs) generated through \textbf{triplet loss} used with Graph transformer &Integration of triplet loss resulted in significant improvements in classification with limited samples and \textbf{demonstrates model's effectiveness in few-shot settings}\\
\hline

 LSTM Attention \& Transformer ~\cite{or2021pay}&	Malware Classification&	Experimented\textbf{ Transformer integrating LSTM} with attentions and without&\textbf{For shorter sequences, LSTM} with attention outperformed Transformers in both accuracy, training time and \textbf{opposite for longer sequences}\\
\hline

Transformer Encoder ~\cite{li2022efficient}	&Malware Classification&MalTransEn leverages \textbf{self-attention} mechanisms for classifying API call sequences&MalTransEn's multi-head self-attention \textbf{efficiently captures interactions} in API call sequences\\
\hline

BERT-based model~\cite{lu2022research}	&Malware Variant Construction and Detection&	\textbf{Pre-trained} on malware API sequences \& \textbf{fine-tuned } by adversarial training for robustness against obfuscation&Adversarial training resulted in \textbf{better} model \textbf{at handling obfuscated API sequences}\\
\hline

\textbf{MDFA}: Bi-LSTM with Attention ~\cite{qi2022mdfa}&	Malware Detection&\textbf{Capture temporal dependencies} in API sequences&	Attention allowed model to \textbf{focus on critical API calls} within long sequences outperforming traditional models\\
\hline

\textbf{B\_ViT} ~\cite{belal2023global}&	Malware Classification&	\textbf{1.} B\_ViT (with Global-Local Attention, Adaptive Positional Encoding) integrates four stages: image partitioning, local attention, global attention, \& classification. Also, enables parallel processing& Significantly \textbf{reduced training time}, with a speed-up factor of 2.42 over IEViT and 1.81 over ViT, \textbf{improved detection} accuracy for \textbf{obfuscated and polymorphic} malware\\
\hline

\textbf{Nebula} ~\cite{trizna2023nebula}	&Malware Detection and Classification&Nebula \textbf{utilizes a self-attention-based} transformer model to process dynamic behavioral reports&Self-attention mechanism allowed Nebula to \textbf{generalize better} across dynamic logs, improving detection accuracy\\
\hline

\textbf{I-MAD:} Galaxy Transformer ~\cite{li2021mad}&	Malware Detection&	Introduced \textbf{3 layer hierarchical Galaxy Transformer} with Satellite-Planet, Planet-Star, and Star-Galaxy transformers to model malware's structure at multiple levels&	\textbf{Reduced time-space complexity} to O(n), enabled model to \textbf{process very long sequences} - previously unmanageable with standard transformer, \textbf{better robustness} for generalization \textbf{to unseen malware}\\
\hline

BERT-CANINE Ensemble~\cite{demirkiran2022ensemble}&Imbalanced Multiclass Malware Classification&\textbf{Introduced} Random Transformer Forest, \textbf{bagging-based ensemble}, with \textbf{fine-tuning} on API call sequences&Ensemble \textbf{improves classification} on \textbf{highly imbalanced datasets}\\

\hline
Transformer and Bi-LSTM ~\cite{chen2020android}&Android malware detection&\textbf{Multi-model architecture} using block feature extraction combined with Multi-Head Attention&Combination of block feature extraction and Multi-Head Attention allowed the model to \textbf{efficiently classify malware}\\
\hline

BERT ~\cite{rahali2021malbert}&	Android malware detection&	\textbf{Fine-tuned} BERT on malware source code with hyperparameter tuning&	Achieved 97.6\% accuracy in binary classification and 91.0\% accuracy in cross-category malware classification\\
\hline

\textbf{SHERLOCK:} ViT with self-supervised learning~\cite{seneviratne2022self}	&Android malware detection &\textbf{Self-supervised} masked autoencoder for \textbf{pre-training}, where 75\% of the pixels in the image were masked and tasked to reconstruct from the unmasked 25\%, then \textbf{fine-tuned} for malware classification &Self-supervised learning approach was \textbf{effective in reducing overfitting}, especially with i\textbf{mbalanced classes} and pre-training enabled to learn robust representations\\

\hline
BERT ~\cite{saracino2023graph}	&Detection and categorization of Android malware&\textbf{Fine-tuned} BERT with data augmentation by manipulating existing sequences to generate new ones, helping to balance the dataset&Able to detect\textbf{ complex malware patterns}\\
\hline

Vision Transformer (ViT) with attention map~\cite{jo2023malware}&	Malware detection and interperability&ViT adapted to take Android app DEX files, converting them into RGB images, generates \textbf{attention map} highlighting specific regions of contributions&Attention maps allows for \textbf{clear visual and textual explanations} of malware detection results\\
\hline

MalBERTv2 (domain specific tokenization)~\cite{rahali2023malbertv2}&	Android Malware Identification&Introduces \textbf{pre-tokenization feature generator} which is trained from scratch on 85,000 Android APK samples and applies to \textbf{fine-tuned BERT}&Code-aware tokenization and fine-tuning proved \textbf{highly effective in multi-class classification}\\
 \hline

 Transformer model with attention~\cite{long2021detecting}&	Android Malware Detection&	Input encoded to 32-dimension with positional encoding \& fed to transformer with 2 attention heads resulting \textbf{small model size} (1.4MB), suitable for mobile&Transformer-based dynamic feature aggregation provided a\textbf{ lightweight yet powerful method} for detecting malware in real-time \textbf{suitable for mobile devices}\\
 \hline
 
 Transformer in Multimodal Network~\cite{dehunting}&	Android malware detection&	Transformer Network (TN) encoder\textbf{ used for temporal feature extractor} from system call sequences in the dynamic analysis subnetwork (Chimera-D)&This adaptation \textbf{reduces noise and captures important temporal patterns }from system call data, leading to more accurate malware detection\\
 \hline

 Heterogeneous Temporal Graph Transformer (HTGT) ~\cite{fan2021heterogeneous}&	Evolving Android malware detection&	HTGT integrates both spatial and temporal dependencies using \textbf{Heterogeneous Spatial Transformer(HST)} for spatial relations among different types of entities and \textbf{Temporal Transformer (TT)} to \textbf{joint model} the malware propagation and evolution through time&	The iterative interaction between HST and TT enhances the ability to \textbf{capture} both \textbf{malware propagation patterns and its evolutionary nature}\\
\hline

BERT ~\cite{ullah2022explainable}&	Android malware detection &	BERT was \textbf{fine-tuned} to extract text features from HTTP and TCP flows, while a malware-to-image conversion technique transformed network byte streams into visual representations for combined feature analysis&\textbf{Combining textual and visual features} allows for a comprehensive analysis of both structural and behavioral malware indicators, \textbf{enhancing detection accuracy}\\
\hline
\end{tabular}%}
\end{adjustbox}
% }
\end{table*}

